Bridging the Bosphorus: Advancing Turkish Large Language Models through Strategies for Low-Resource Language Adaptation and Benchmarking

Large Language Models (LLMs) are becoming crucial across various fields, emphasizing the urgency for high-quality models in underrepresented languages. This study explores the unique challenges faced by low-resource languages, such as data scarcity, model selection, evaluation, and computational limitations, with a special focus on Turkish. We conduct an in-depth analysis to evaluate the impact of training strategies, model choices, and data availability on the performance of LLMs designed for underrepresented languages. Our approach includes two methodologies: (i) adapting existing LLMs originally pretrained in English to understand Turkish, and (ii) developing a model from the ground up using Turkish pretraining data, both supplemented with supervised fine-tuning on a novel Turkish instruction-tuning dataset aimed at enhancing reasoning capabilities. The relative performance of these methods is evaluated through the creation of a new leaderboard for Turkish LLMs, featuring benchmarks that assess different reasoning and knowledge skills. Furthermore, we conducted experiments on data and model scaling, both during pretraining and fine-tuning, simultaneously emphasizing the capacity for knowledge transfer across languages and addressing the challenges of catastrophic forgetting encountered during fine-tuning on a different language. Our goal is to offer a detailed guide for advancing the LLM framework in low-resource linguistic contexts, thereby making natural language processing (NLP) benefits more globally accessible.

==> imgs/abstract.tex <==
As Large Language Models (LLMs) become increasingly integral in various domains, the need for high-quality models in underrepresented languages becomes more pressing.
In this study, we explore the adaptation and performance of LLMs for Turkish, a representative of low-resource languages, through two distinct methodologies: (i) adapting a high-performing monolingual base model, initially trained in English, to learn Turkish, (ii) training a model entirely from scratch in GPT2 scales. The resulting models are further refined using supervised fine-tuning with a newly created instruction dataset to better align them with the specific response traits or domain knowledge. 
Finally, recognizing the scarcity of resources for evaluating reasoning and world knowledge capabilities for LLMs in Turkish, we created two novel Turkish QA evaluation benchmarks Turkish-TruthfulQA and ARC-tr.
Our study not only presents a novel solution for Turkish language processing but also establishes a framework for developing LLMs in other low-resourced languages, demonstrating the potential of LLMs for languages other than English.


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> plots/case_studies_4_1.tex <==
\begin{figure}[!htb]
\centering
\begin{tikzpicture}
    \begin{axis}[
        title={Accuracy Comparison of Hamza Models on Turkish QA Tasks},
        xlabel={Data Size (GB)},
        ylabel={Accuracy (ARC-TR)},
        xmin=0, xmax=6,
        ymin=20, ymax=45,
        xtick={0.1, 0.25, 0.5, 1, 2, 5},
        xticklabels={$\frac{1}{10}$, $\frac{1}{4}$, $\frac{1}{2}$, 1, 2, 5},
        ytick={20, 25, 30, 35, 40, 45},
        legend pos=outer north east,
        legend style={at={(0.99,0.92)},anchor=east},
        legend cell align={left},
        ymajorgrids=true,
        grid style=dashed,
        enlarge x limits=false,
        tick label style={font=\small},
        label style={font=\small},
        width=0.7\textwidth,
    ]

    \addplot[
        color=blue,
        mark=square,
        thick,
        ]
        coordinates {
        (0.1, 24.91)(0.25, 23.46)(0.5, 24.66)(1, 24.66)(2, 25.09)(5, 24.49)
        };
        \addlegendentry{GPT2-xl}

    \addplot[
        color=red,
        mark=triangle,
        thick,
        ]
        coordinates {
        (0.1, 35.27)(0.25, 37.37)(0.5, 37.03)(1, 38.57)(2, 39.85)(5, 40.70)
        };
        \addlegendentry{Mistral}
        
    \end{axis}
\end{tikzpicture}
\caption{Performance of our models: pretrained Hamza models with different sizes, and the Hamza$_{\scriptsize Mistral}$ and Hamza$_{\scriptsize GPT2-xl}$ models that are adapted on Turkish. We present the result of our ablation study evaluated on the ARC-TR and TruthfulQA-TR datasets, where the performance of the adapted models is given by progressively enlarging the pretraining corpus size from 0.1GB to 5GB.}
\label{fig:models-accuracy}
\end{figure}

==> plots/case_studies_4_4.tex <==

\begin{figure}[!htb]
\centering
\begin{tikzpicture}
\begin{axis}[
    title={\textbf{Comparison of ARC Scores by Language}},
    xlabel={\textbf{\# of Turkish Tokens Mistral 7B Continued Pretrained on}},
    ylabel={\textbf{\textcolor{red}{English} \&  \textcolor{blue}{Turkish} ARC Acc.}},
    xtick={0,1,2,3,4,5,6},
    xticklabels={
        0,
        50M,
        130M,
        250M,
        0.5B,
        1.1B,
        2.5B,
    },
    xlabel style={at={(0.5,-0.10)}},
    legend pos=outer north east,
    ymajorgrids=true,
    grid style=dashed,
    legend style={cells={align=left}},
    width=0.7\textwidth,
    xtick distance=3,
    legend style={at={(0.99,0.91)},anchor=east},
]

% Adding data for Turkish ARC
\addplot[
    color=blue,
    mark=o,
    thick,
    nodes near coords,
    point meta=explicit symbolic,
] coordinates {
    (0,33.11)
    (1,35.27)
    (2,37.37)
    (3,37.03)
    (4,38.57)
    (5,39.85)
    (6,40.70)
};

% Adding data for English ARC
\addplot[
    color=red,
    mark=square,
    thick,
    nodes near coords,
    point meta=explicit symbolic,
] coordinates {
    (0,60.41)
    (1,56.06)
    (2,52.39)
    (3,52.39)
    (4,51.71)
    (5,49.40)
    (6,46.76)
};

\legend{ARC-tr Acc., ARC-eng Acc.}
\end{axis}
\end{tikzpicture}
\caption{Mistral performance on Turkish and English ARC tasks.}
\end{figure}





==> tables/bpc_evaluation.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{Models}         &\textbf{}                   &\textbf{PPL per token}          &\textbf{Model Size (B)}         &\textbf{TrNews-64 BPC}   \\ \midrule
kanarya-2b              & -                          & 13.684                      & 2.06                     & \textbf{0.724}          \\
kanarya-750m            & -                          & 11.846                      & 0.74                     & 0.767                   \\
xglm-7.5B               & -                          & 12.184                      & 7.49                     & 0.880                   \\
xglm-4.5B               & -                          & 14.821                      & 4.55                     & 0.949                   \\
xglm-2.9B               & -                          & 14.723                      & 2.94                     & 0.946                   \\ 
xglm-1.7B               & -                          & 19.418                      & 1.73                     & 1.044                   \\ 
xglm-564M               & -                          & 24.503                      & 0.56                     & 1.125                   \\ 
mGPT                    & -                          & 16.490                      & 1.42                     & 1.306                   \\ 
ytu-gpt2-large          & -                          & 2224041771.471              & 0.77                     & 6.058                   \\
Trendyol-7b-chat        & -                          & 9.461                       & 6.84                     & 0.820                   \\
Trendyol-7b-base        & -                          & 9.714                       & 6.84                     & 0.829                   \\
LLaMA2-7b               & -                          & 6.929                       & 6.74                     & 1.374                   \\
LLaMA2-7b-chat          & -                          & 11.109                      & 6.74                     & 1.709                   \\
Mistral-7b              & -                          & 5.733                       & 7.24                     & 1.260                   \\
Mistral-7b-chat         & -                          & 10.002                      & 7.24                     & 1.662                   \\
Mixtral-8x7b            & -                          & 4.564                       & 46.70                    & 1.096                   \\
gemma-2B-tr             & -                          & 12.591                      & 2.51                     & 1.089                   \\ 
gemma-2B                & -                          & 16.613                      & 2.51                     & 1.208                   \\
gemma-7B                & -                          & 9.974                       & 8.54                     & 0.989                   \\
gpt2-xl                 & -                          & 34.139                      & 1.56                     & 2.533                   \\ 

%Hamza-s                 & 25.60                      & 26.37                       & 43.52                    & 0.897           \\
%Hamza-m                 & 27.99                      & 25.77                       & 42.48                    & 0.814           \\
%Hamza-l                 & 29.52                      & 29.10                       & 40.11                    & 0.760           \\
%Hamza-xl                & 29.69                      & 27.99                       & 39.47                    & 0.754*           \\ \midrule
%Mistral + our 2GB       & \textbf{39.85}            & \textbf{34.81}               & 42.72                    & TODO           \\ 
\bottomrule
\end{tabular}

\caption{Perplexity per token and Bits-Per-Character (BPC) results, model sizes }
\label{tab: acc-results}
\end{table*}

% Ya Tğürkçe converge olmadı
% Türkçe öğretirken science'ı unutturduk mu, türkçe-finetuned'a bir daha ingilizce bakalım.
% Science'ı ingilizce'den türkçeye çevirmeyi

%METE Questions
% TR-New BPC -> TrNews-64 BPC?
% Mistral-7b-chat  or  Mistral-7b-instruct?





==> tables/case_studies_4_1.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{} & \multicolumn{3}{c}{\textbf{Accuracy ($\uparrow$)}} &\textbf{} \\ \cmidrule(lr){2-5} 
\textbf{Models}         &\textbf{ARC-TR}   &\textbf{ARC-TR}     &\textbf{TruthfulQA-TR}    &\textbf{Avg.}  \\
\textbf{}              &\textbf{(25-shot)} &\textbf{(0-shot)}     &\textbf{}    &\textbf{}         \\ \midrule
Hamza-small                                & 25.60             & 26.37       & 43.45      & 31.8           \\
Hamza-medium                               & 27.99             & 25.77       & 42.17      & 32.0           \\
Hamza-large                                & 29.52             & 29.10       & 39.97      & 32.9           \\
Hamza-xlarge                               & 29.69             & 27.99       & 39.69      & 32.5           \\ \midrule
Hamza$_{\scriptsize GPT2-xl}$ (0.1GB)        & 24.91             & 24.49       & 48.36      & 32.6           \\  
Hamza$_{\scriptsize GPT2-xl}$ (0.25GB)       & 23.46             & 24.57       & 47.16      & 31.7           \\  
Hamza$_{\scriptsize GPT2-xl}$ (0.5GB)        & 24.66             & 23.04       & 46.52      & 31.4           \\  
Hamza$_{\scriptsize GPT2-xl}$ (1GB)          & 24.66             & 24.15       & 45.32      & 31.4           \\  
Hamza$_{\scriptsize GPT2-xl}$ (2GB)          & 25.09             & 24.57       & 45.54      & 31.7           \\
Hamza$_{\scriptsize GPT2-xl}$ (5GB)          & 24.49             & 23.72       & 45.34      & 31.2           \\ \midrule
Hamza$_{\scriptsize Mistral}$ (0.1GB)        & 35.27             & 29.95       & 43.26      & 36.2           \\ 
Hamza$_{\scriptsize Mistral}$ (0.25GB       & 37.37             & 32.25       & 44.08      & 37.9           \\ 
Hamza$_{\scriptsize Mistral}$ (0.5GB)        & 37.03             & 31.40       & 42.04      & 36.8           \\ 
Hamza$_{\scriptsize Mistral}$ (1GB)          & 38.57             & 31.91       & 44.67      & 38.4           \\ 
Hamza$_{\scriptsize Mistral}$ (2GB)          & 39.85             & 34.81       & 44.05      & 39.6           \\
Hamza$_{\scriptsize Mistral}$ (5GB)         & 40.70             & 36.01       & 44.44      & 40.4           \\ \bottomrule
\end{tabular}

\caption{\textbf{Accuracy comparison of our models on Turkish question answering tasks.} This table shows the performance of our models: pretrained Hamza models with different sizes, and the Hamza$_{\scriptsize Mistral}$ and Hamza$_{\scriptsize GPT2-xl}$ models that are adapted on Turkish. We present the result of our ablation study evaluated on the ARC-TR and TruthfulQA-TR datasets, where the performance of the adapted models are given by progressively enlarging the pretraining corpus size from 0.1GB to 5GB. }
\label{tab: case-studies-4-1}
\end{table*}

==> tables/case_studies_4_3.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{Models}     &\textbf{LLaMA2 7b}  &\textbf{Mistral 7b}  &\textbf{Hamza-xl}  &\textbf{Kanarya-7b}      \\ \midrule
ARC (25-shot)       & 52.99              & 60.41               & 19.45             & 23.21                   \\
ARC-tr (25-shot)    & 27.47              & 33.11               & 29.69             & 32.08                   \\
TruthfulQA          & 38.97              & 42.58               & 46.84             & 40.66                   \\
TruthfulQA-tr       & 41.85              & 41.93               & 39.47             & 39.38                   \\ 
\bottomrule
\end{tabular}
\caption{Cross-lingual Transfer}
\label{tab: case-studies-4-3}
\end{table*}

==> tables/case_studies_4_4.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{Models}                            &\textbf{ARC}                        &\textbf{TruthfulQA}       &\textbf{Avg.}   \\ \midrule
GPT2-xl                                    & 30.29                              & 38.53                    & 34.41           \\ 
Hamza$_{\scriptsize GPT2-xl}$ (0.1GB)      & 27.82                              & 38.15                    & 32.98           \\
Hamza$_{\scriptsize GPT2-xl}$ (0.25GB)     & 27.65                              & 38.10                    & 32.88           \\
Hamza$_{\scriptsize GPT2-xl}$ (0.5GB)      & 27.82                              & 38.88                     & 33.35           \\
Hamza$_{\scriptsize GPT2-xl}$ (1GB)        & 27.22                              & 38.95                     & 33.09           \\
Hamza$_{\scriptsize GPT2-xl}$ (2GB)        & 25.68                              & 40.34                     & 33.01           \\
Hamza$_{\scriptsize GPT2-xl}$ (5GB)        & 23.63                              & 41.36                     & 32.49           \\ \midrule
Mistral-7b                                 & 60.41                              & 42.58                   & 51.49           \\ 
Hamza$_{\scriptsize Mistral}$ (0.1GB)      & 56.06                              & 40.37                   & 48.22           \\
Hamza$_{\scriptsize Mistral}$ (0.25GB)     & 52.39                              & 39.14                   & 45.77           \\
Hamza$_{\scriptsize Mistral}$ (0.5GB)      & 52.39                              & 38.63                   & 45.51           \\
Hamza$_{\scriptsize Mistral}$ (1GB)        & 51.71                              & 41.49                   & 46.60           \\
Hamza$_{\scriptsize Mistral}$ (2GB)        & 49.40                              & 38.42                   & 43.91           \\
Hamza$_{\scriptsize Mistral}$ (5GB)        & 46.76                              & 40.88                   & 43.82           \\ \bottomrule
\end{tabular}
\caption{\textbf{Accuracy comparison of our models on English question answering tasks.} This table shows the performance of our Hamza$_{\scriptsize Mistral}$ and Hamza$_{\scriptsize GPT2-xl}$ models that are adapted on Turkishi together with the original Mistral-7b and GPT2-xl. We present the result of our ablation study, where the performance of the adapted models is given by progressively enlarging the pretraining corpus size from 0.1 GB to 5 GB. Here, the zero and few-show accuracies are evaluated on the original ARC and TruthfulQA. }
\label{tab: case-studies-4-4}
\end{table*}

==> tables/evaluation.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{clcccc}
\toprule
\textbf{}               & \textbf{}                  & \multicolumn{3}{c}{\textbf{Accuracy ($\uparrow$)}} &\textbf{BPC ($\downarrow$)} \\ \cmidrule(lr){3-5} \cmidrule(lr){6-6}
\textbf{Type}               &\textbf{Models}         &\textbf{ARC-TR}             &\textbf{ARC-TR}              &\textbf{Truthful-}    &\textbf{\textsc{trnews-64}}   \\
\textbf{}               &\textbf{}               &\textbf{(25-shot)}          &\textbf{(0-shot)}            &\textbf{QA-TR}                 &\textbf{}              \\ \midrule

\multirow{7}{*}{\shortstack[l]{\textbf{Base} \\ \textbf{and SFT} \\ \textbf{Models}}} 
& LLaMA2-7b               & 27.47                      & 25.77                       & 41.51                    & 1.374                 \\
& Mistral-7b              & 33.11                      & 30.20                       & 42.55                    & 1.260                 \\
& Gemma-2B                & 24.91                      & 23.63                       & 42.04                    & 1.208                 \\
& Gemma-7B                & 24.91                      & 25.77                       & 47.17                    & 0.989                 \\
& GPT2-xl                 & 24.91                      & 25.17                       & 40.97                    & 2.533                 \\ 
& Mistral-7b-chat-v2      & 35.24                      & 29.27                       & \underline{48.34}        & 1.428                 \\ \midrule

\multirow{6}{*}{\shortstack[l]{\textbf{Multi-} \\ \textbf{lingual} \\ \textbf{Models}}} 
& XGLM-7.5B               & 30.29                      & 28.41                       & 38.38                    & 0.880                 \\
& XGLM-4.5B               & 29.01                      & 27.47                       & 40.34                    & 0.949                 \\
& XGLM-2.9B               & 28.41                      & 27.30                       & 40.03                    & 0.946                 \\ 
& XGLM-1.7B               & 28.24                      & 25.51                       & 40.97                    & 1.044                 \\ 
& XGLM-564M               & 25.00                      & 23.98                       & 42.00                    & 1.125                 \\ 
& mGPT                    & 27.30                      & 24.57                       & 41.34                    & 1.306                 \\ \midrule

\multirow{11}*{\shortstack[l]{\textbf{HF} \\ \textbf{Turkish} \\ \textbf{Models}}} 
& Kanarya-2b              & 32.08                      & 29.35                       & 40.49                    & \textbf{0.724}                 \\
& Kanarya-750m            & 30.12                      & 27.30                       & 41.24                    & 0.767                 \\
& ytu-gpt2-large          & 27.99                      & 26.28                       & 42.90                    & 0.805                 \\
& Trendyol-7b-base        & 35.24                      & 30.38                       & 41.50                    & 0.829                 \\
& Trendyol-7b-chat        & 35.58                      & 30.63                       & 44.35                    & 0.820                 \\
& Trendyol-7b-dpo         & \textbf{40.78}             & \underline{34.73}           & \textbf{49.57}           & 0.859                 \\
%& Commencis-LLM           & 34.13                      & 29.95                       & 45.79                    & 1.306                 \\
%& Sambalingo-tr           & 44.71                      & 38.31                       & 42.07                    & 0.894                 \\
& Thestral-tr-chat        & 33.70                      & 31.40                       & 42.36                    & 1.314                 \\ 
& Mistral-7b-chat-v2-tr   & 34.98                      & 29.44                       & 46.13                    & 1.411                 \\
& Gemma-2B-tr             & 31.23                      & 27.22                       & 43.54                    & 1.089                 \\ \midrule

\multirow{6}{*}{\textbf{\shortstack[l]{\textbf{Our} \\ \textbf{Models}}}} 
& Hamza-small             & 25.60                      & 26.37                       & 43.45                    & 0.897                 \\
& Hamza-medium            & 27.99                      & 25.77                       & 42.17                    & 0.814                 \\
& Hamza-large             & 29.52                      & 29.10                       & 39.97                    & 0.760                 \\
& Hamza-xlarge            & 29.69                      & 27.99                       & 39.69                    & \underline{0.754}     \\ 
& Hamza$_{\scriptsize GPT2-xl}$  & 24.49               & 23.72                       & 45.34                    & 1.152                 \\  
& Hamza$_{\scriptsize Mistral}$  & \underline{40.70}    & \textbf{36.01}              & 44.44                    & 0.816                 \\ 

\bottomrule
\end{tabular}

\caption{\textbf{Performance comparison on various Turkish tasks.} In this table we compare the performance of various types of models: (i) Base and SFT Models, (ii) Multilingual Models (iii) Open-Source HF (Huggingface) Turkish Models, (iv) Our pretrained and adopted Hamza Models. The first three column shows zero and few-show accuracies evaluated on the ARC-TR and TruthfulQA-TR datasets. The last column includes the Bits-Per-Character (BPC) metric evaluated on \textsc{trnews-64} corpus. Note that Accuracy is the highest and BPC is the lowest for the best models. The top-performing model for each metric is highlighted in bold, while the second-best model is underlined for easy identification.}
\label{tab: acc-results}
\end{table*}

% Ya Tğürkçe converge olmadı
% Türkçe öğretirken science'ı unutturduk mu, türkçe-finetuned'a bir daha ingilizce bakalım.
% Science'ı ingilizce'den türkçeye çevirmeyi

% TR-New BPC -> TrNews-64 BPC





==> tables/gemma-todos.tex <==
\begin{table*}[!t]
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccccccccc}
\hline
\textbf{Model} & \textbf{Dataset Size} & \textbf{Batch Size} & \textbf{M. Batch Size}   & \textbf{LR}     & \textbf{Target Modules}           & \textbf{Rank}      & \textbf{Alpha}   & \textbf{Train Loss}  & \textbf{Val Loss}   \\ \toprule
gemma 7b        & 0.1GB                & 1                   & 1                        & 1.0$e^{-4}$     & \{gate, up, down\}\_proj          & 32                 & 32               & TODO                 & TODO              \\ 
gemma 7b        & 0.25GB                & 1                   & 1                        & 1.0$e^{-4}$     & \{gate, up, down\}\_proj         & 32                 & 32               & TODO                 & TODO              \\ 
gemma 7b        & 0.5GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{gate, up, down\}\_proj         & 32                 & 32               & TODO                 & TODO              \\ 
gemma 7b        & 1.0GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{gate, up, down\}\_proj         & 32                 & 32               & TODO                 & TODO              \\ 
gemma 7b        & 2.5GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v\}\_proj                   & 32                 & 32               & TODO                 & TODO               \\ 
gemma 7b        & 5.0GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v\}\_proj                   & 32                 & 32               & TODO                 & TODO               \\ 
gemma 7b        & 10.0GB                & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v\}\_proj                   & 32                 & 32               & TODO                 & TODO               \\  \bottomrule
\end{tabular}
}
\caption{ gemma continued pretraining ablation experiments.}
\label{tab: gemma}
\end{table*}


==> tables/gpt2-todos.tex <==
\begin{table*}[!t]
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccccccccc}
\hline
\textbf{Model} & \textbf{Dataset Size} & \textbf{Batch Size} & \textbf{M. Batch Size}   & \textbf{LR}     & \textbf{Target Modules}          & \textbf{Rank}      & \textbf{Alpha}   & \textbf{Train Loss}  & \textbf{Val Loss}   \\ \toprule
gpt2-xl        & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{att\}\_proj                    & 32                 & 32               & 3.130                 & 2.000              \\
gpt2-xl        & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{proj\}\_proj                   & 32                 & 32               & 2.643                 & 1.686              \\
gpt2-xl        & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{att,proj\}\_proj               & 32                 & 32               & 2.653                 & 1.704              \\ 
gpt2-xl        & 0.1GB                 & 2                   & 8                        & 1.0$e^{-4}$     & \{att,proj\}\_proj               & 32                 & 32               & 11.466                 & TODO               \\ \midrule


gpt2-xl        & 0.25GB                & 1                   & 1                        & 1.0$e^{-4}$     & \{proj\}\_proj                   & 32                 & 32               & 2.643                 & 1.547              \\ 
gpt2-xl        & 0.5GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{proj\}\_proj                   & 32                 & 32               & 2.199                 & 1.386              \\ 
gpt2-xl        & 1.0GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{proj\}\_proj                   & 32                 & 32               & TODO                 & TODO              \\ 
gpt2-xl        & 2.5GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{proj\}\_proj                   & 32                 & 32               & TODO                 & TODO               \\ 
gpt2-xl        & 5.0GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{proj\}\_proj                   & 32                 & 32               & TODO                 & TODO               \\ 
gpt2-xl        & 10.0GB                & 1                   & 1                        & 1.0$e^{-4}$     & \{proj\}\_proj                   & 32                 & 32               & TODO                 & TODO               \\  \bottomrule
\end{tabular}
}
\caption{ gpt2 continued pretraining ablation experiments.}
\label{tab: gpt2}
\end{table*}
% 2.5351905822753906

==> tables/mistral-todos.tex <==
\begin{table*}[!t]
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccccc}
\hline
\textbf{Model} & \textbf{Dataset Size} & \textbf{Batch Size} & \textbf{M. Batch Size}   & \textbf{LR}     & \textbf{Target Modules}          & \textbf{Rank}      & \textbf{Alpha}   & \textbf{Train Loss}  & \textbf{Val Loss}   \\ \toprule
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 5.0$e^{-3}$     & \{q, v\}\_proj                   & 8                  & 16               & 6.430                & 4.320              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-3}$     & \{q, v\}\_proj                   & 8                  & 16               & 1.986                & 1.420              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 6.0$e^{-4}$     & \{q, v\}\_proj                   & 8                  & 16               & 1.836                & 1.208              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v\}\_proj                   & 8                  & 16               & 1.750                & 1.197              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 5.0$e^{-5}$     & \{q, v\}\_proj                   & 8                  & 16               & 1.759                & 1.210              \\ \midrule
Mistral-7B     & 0.1GB                 & 8                   & 2                        & 1.0$e^{-3}$     & \{q, v\}\_proj                   & 8                  & 16               & 1.774                & 1.238              \\ 
Mistral-7B     & 0.1GB                 & 8                   & 2                        & 6.0$e^{-4}$     & \{q, v\}\_proj                   & 8                  & 16               & 1.778                & 1.245              \\
Mistral-7B     & 0.1GB                 & 8                   & 2                        & 1.0$e^{-4}$     & \{q, v\}\_proj                   & 8                  & 16               & 1.807                & 1.277              \\
Mistral-7B     & 0.1GB                 & 8                   & 2                        & 5.0$e^{-5}$     & \{q, v\}\_proj                   & 8                  & 16               & 1.816                & 1.284              \\ \midrule
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v\}\_proj                   & 8                  & 16               & 1.750                & 1.197              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v\}\_proj                   & 16                 & 16               & 1.731                & 1.176              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v\}\_proj                   & 32                 & 32               & 1.710                & 1.149              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v\}\_proj                   & 64                 & 64               & 1.694                & 1.127              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v\}\_proj                   & 128                & 128              & 1.687                & 1.107              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{gate, up, down\}\_proj         & 8                  & 16               & 1.623                & 1.067              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{gate, up, down\}\_proj         & 16                 & 16               & 1.588                & 1.037              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{gate, up, down\}\_proj         & 32                 & 32               & 1.572                & 1.013              \\ 
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{gate, up, down\}\_proj         & 64                 & 64               & 1.571                & 1.000              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{gate, up, down\}\_proj         & 128                & 128              & 1.596                & 0.999              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v, gate, up, down\}\_proj   & 8                  & 16               & 1.623                & 1.062              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v, gate, up, down\}\_proj   & 16                 & 16               & 1.587                & 1.032              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v, gate, up, down\}\_proj   & 32                 & 32               & 1.575                & 1.011              \\
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v, gate, up, down\}\_proj   & 64                 & 64               & 1.580                & 1.002              \\ 
Mistral-7B     & 0.1GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v, gate, up, down\}\_proj   & 128                & 128              & 1.616                & 1.009              \\ \midrule
Mistral-7B     & 0.25GB                & 1                   & 1                        & 1.0$e^{-4}$     & \{gate, up, down\}\_proj         & 32                 & 32               & 1.528                & 0.973              \\ 
Mistral-7B     & 0.5GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{gate, up, down\}\_proj         & 32                 & 32               & 1.501                & 0.949              \\ 
Mistral-7B     & 1.0GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{gate, up, down\}\_proj         & 8                  & 16               & 1.478                & 0.930              \\ 
Mistral-7B     & 2.5GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v\}\_proj                   & 8                  & 16               & TODO                 & TODO               \\ 
Mistral-7B     & 5.0GB                 & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v\}\_proj                   & 8                  & 16               & TODO                 & TODO               \\ 
Mistral-7B     & 10.0GB                & 1                   & 1                        & 1.0$e^{-4}$     & \{q, v\}\_proj                   & 8                  & 16               & TODO                 & TODO               \\  \bottomrule
\end{tabular}
}
\caption{ Mistral continued pretraining ablation experiments.}
\label{tab: mistral}
\end{table*}

